rIoT: Enabling Seamless Context-Aware Automation in the Internet of Things

Advances in mobile computing capabilities and an increasing number of Internet of Things (IoT) devices have enriched the possibilities of the IoT but have also increased the cognitive load required of IoT users. Existing context-aware systems provide various levels of automation in the IoT. Many of these systems adaptively take decisions on how to provide services based on assumptions made a priori. The approaches are difficult to personalize to an individual's dynamic environment, and thus today's smart IoT spaces often demand complex and specialized interactions with the user in order to provide tailored services. We propose rIoT, a framework for seamless and personalized automation of human-device interaction in the IoT. rIoT leverages existing technologies to operate across heterogeneous devices and networks to provide a one-stop solution for device interaction in the IoT. We show how rIoT exploits similarities between contexts and employs a decision-tree like method to adaptively capture a user's preferences from a small number of interactions with the IoT space. We measure the performance of rIoT on two real-world data sets and a real mobile device in terms of accuracy, learning speed, and latency in comparison to two state-of-the-art machine learning algorithms.

==> previous_writing.tex <==
An essential component of a user interacting with smart environment is determining which smart thing(s) in the environment should be leveraged to support a user's intentional interactions. For example, when a user flips a light switch, which light should turn on? When a user opens a video feed for information along his path, which camera should be used? When the user wants to open the blinds, lock the door, change the thermostat, play some music, ..., which blinds, lock, thermostat, and speakers should be used?

Using current systems, users are expected to navigate lists of smart devices with semantic descriptions that help the users explicitly select the appropriate smart devices to use. This also entails significant setup and configuration costs on the user's part: when a new device is added to a space, someone must explicitly name and describe it, in a way that is accessible to anyone else who might use the device. While this might be straightforward in a home with a small number of users, when extended to a larger or more public space, semantic labeling becomes quite challenging.

In this paper, we investigate techniques for selecting things for users' tasks in ways that \textit{do not} require significant set up costs. 

A na\"{i}ve first step, and one explored in the literature, is to assume the user wants to use the ``closest'' device with the needed capability.
\begin{itemize}
    \item [+] simple to implement and understand
    \item [+] matches a majority of use cases
    \item [-] requires fine-grained localization of devices, which can be quite difficult indoors
    \item [-] does not match several common use cases and situations
\end{itemize}
As an example of the latter, this cannot address situations where the closest device doesn't ``cover'' the target location of the action. For instance, the closest smart light might be behind a closed door; the closest camera might be pointed in the wrong direction, etc.

To address this challenge, we can recognize that many smart devices have {\em physical scopes}.\footnote{Does a lock have a reasonable physical scope? If not, should we include it above? How about blinds?} An obvious iteration of the above first step is to select the closest thing whose physical scope includes the ``target location'' (which may or may not be the user's location).
\begin{itemize}
    \item [+] continues to match a majority of use cases
    \item [+] addresses the concern with na\"{i}ve ``closest'' selection
    \item [-] still requires fine grained locations of all devices
    \item [-] requires smart devices to be pre-programmed with their physical scopes 
\end{itemize}
This last point greatly increases the setup burden of the smart space.

A third step allows the smart devices to {\em learn} their physical scopes over time based on successful (or unsuccessful) interactions with users. This requires introducing an {\em interaction history} that logs these successes and failures over time.
\begin{itemize}
    \item [+] continues to address a majority of use cases
    \item [+] dramatically reduces setup costs (devices can be deployed with a default physical scope that changes as it learns)
    \item [-] still requires fine-grained locations of all devices
    \item [-] is more complicated, especially because it requires addressing privacy concerns related to storing and mixing multiple users' interaction histories
\end{itemize}
We address the latter concern through options that allow an interaction history to be made private (i.e., stored only on a user's personal device) or made public (i.e., stored at the smart device itself). These options tradeoff privacy for the speed at which a device can learn its physical scope.

  A final iteration could recognize that fine-grained location is not really necessary; rather what is used is the relative location of a user and the smart devices in the environs.\footnote{\color{red}We didn't talk about this, but integrating the RSSI stuff that Sarnab and Rebecca did could help us here. Thoughts?}
\begin{itemize}
    \item [+] continues to address a majority of use cases
    \item [+] dramatically reduces setup costs (devices can be deployed with a default physical scope that changes as it learns)
    \item [+] removes the need for fine-grained localization
    \item [-] increases complexity of installation and implementation because it demands the ability to use wireless signals as a proxy for localization
\end{itemize}


==> related_works.tex <==
\section{Related Work and Background}\label{sec:related_works}


% \tocheckCL{
% \begin{itemize}
%   \item Automated recommendation based on primitive(also effective) information: who and where~\cite{salber1999context}. More advanced ways like situational awareness could also be mentioned. 
%   \item Control smart devices using manually created polices~\cite{sun2015efficient}, IFTTT~\cite{mi2017empirical} and actuators~\cite{sun2013multi}
%   \item Automation of deriving policies and device selection.
% \end{itemize}
% }

\note{You should add something here, even if just one sentence to describe the subsections of this section.}\cj{Just a general, updated comment about the related work: it really just reads as a list of projects with brief descriptions. I think perhaps because the real research problem and intended contributions are not as clear from the introduction, it's hard to relate these comments to what you intend to do. Is it possible to frame/organize this related work section to some how mirror the order/contents of the (revised) list of contributions in the introduction?}

\subsection{Context-Awareness in the IoT}\cj{Is this a title that encompasses {\em all} of the relevant related work? What about middleware for simplifying IoT interactions that are {\em not} context-aware? Are there any machine learning approaches for interaction int the IoT that might not be considered context-aware?}
Due to advance\tocheckCJ{s} in \tocheckCJ{\sout{mobile device}} technology, IoT devices are \tocheckCJ{\sout{becoming}} more powerful\cj{What does powerful mean in this context?}, cost less, and have more communication capabilities. As a result, a large number of devices are deployed today, and it is predicted that the number will grow rapidly in the following years~\cite{whitmore2015internet}. On one hand, more low-power sensors can provide continuous, real-time contextual data about the user,
% \cj{Always a comma before which, never a comma before that.}
which enables more\cj{more than what?} expressive context-aware applications. On the other hand, it is not feasible for an individual user to individually connect to and control the devices in a one-by-one manner. The need for context-awareness has not only been identified in the research community~\cite{sezer2018context} but also by the IoT industry~\cite{da2014internet}. Context-awareness techniques can leverage data collected by  sensors in the environment and the devices available by the user in a non-static way which is essential in mobile devices setting.\cj{This last part of the sentence doesn't parse well for me. What are you trying to say? Also, at this point it strikes me that up to this point in the paper, there's not a concrete example of how context could be used. Perhaps a scenario preceding this related work section (but as part of Section 2) would be beneficial. I wrote this comment before I read Section 3. I'm still not sure that we don't need the example earlier. I might consider combining Sections 2 and 3, with the meat of Section 3 actually coming first. You could even use what is currently Section 3.1 to help frame the related work discussion (TBH, the contents of Section 3.1 are also ``related work'', and kind of address my first comment in this section as well).} 

% Early solutions\cj{To what? Early solutions to using context information to influence interaction in the IoT?} like~\cite{salber1999context} use only basic context information, e.g., such as identity and location to provide automated recommendation\cj{This seems like an oxymoron. I've been thinking that ``automation'' means that the system will do something on the user's behalf. This seems to be talking about recommendation. Recommendation for what? Then I would be careful about being ``loose'' with the term automation. Further, is it a distinguishing feature for our approach that we DO automation, whereas these other approaches did only recommendation?}. 
Several existing works adopt a semantic approach~\cite{kao2012user,maarala2017semantic,sun2015efficient,gu2004ontology} where the context-awareness is based on pre-defined ontology of device, user and environment. Unlike these approaches, \systemname does not require a priori information how each devices affect the space which makes it suitable for dynamic and personal space for which the ontology is not available. CA4IOT~\cite{perera2013context,perera2012ca4iot} is a context-aware architecture for sensor selection based on the likelihood index from the weighted euclidean distance from the user's context and the context of the sensors. However, the context reasoning is only based on static distance function with pre-defined context-type. Probabilistic and association based solutions~\cite{nath2012ace,luxey2018sprinkler} have been proposed to help provide efficient activity sensing and fluid device interaction. Some other works~\cite{chahuara2013making,chahuara2017context,chen2016context,mannini2010machine,ruvzic2014context} use Hidden Markov Model(HMM) to model context-awareness. These approaches either require a list of pre-defined ``situations'', or some assumptions on the ontology of context and environment. More deep machine learning approaches are brought into the fields of context-aware activity recognition, interaction prediction, and smart space automation~\cite{radu2018multimodal, ordonez2016deep, hammerla2016deep}. Despite the promising accuracy, deep learning approaches require enormous data points, which makes it not suitable for personalized space that does not generate enough data. 

% \textit{Sprinkler}~\cite{luxey2018sprinkler}, ACE~\cite{nath2012ace}, \cite{radu2018multimodal} and \cite{chahuara2013making} share a data-driven view of context-awareness as we do in \systemname. \textit{Sprinkler} builds a Markov model from user interaction history to predict the next device that the user want to use. The framework focuses on providing convenience instead of automation which makes it not suitable for our use case. ACE and \cite{radu2018multimodal} are two parallel work focusing on using contextual information to provide better activity recognition. ACE uses association rule mining to make the  activity sensing more efficiently while Radu uses deep learning method to accurately recognize human activity. In \cite{chahuara2013making,chahuara2017context}, the authors proposed a decision making framework with focus on {\em context-awareness}. The goal is similar to ours as determining the right device to perform an IoT action given a user request. Yet the approach is using a Markov Logic Network (MLN) , which is built on a list of pre-defined ``situations'', to learn the user's preference of a lighting system. While in this work we broaden the use of context-awareness and mitigate the need on specifying the circumstances of interest as from their approach. 
% \note{Machine learning approaches}

The aforementioned approaches inspired our work, though we target a more general space with different device types and dynamic changing. The key challenges of \textit{interactive machines in general} as identified by Suchman~\cite{suchman2007human} articulate a gap between what computing systems can sense and the user's intentions. That is, no matter how many sensors we include, there will be gaps in the system's knowledge. Therefore, unlike most existing solutions, we emphasize that user's feedback should be include explicitly into learning process.

\subsection{Preliminaries of \systemname}
\note{Sensor Network: efficiently and continuously provide rich context information (conmon, stacon)}
Efficiently collecting or sharing context information from sensors have been well studied in the field of Wireless Sensor Network(WSN). Given the increased wide variety of sensor modalities available in recent years, there is a trend of research efforts focusing on building context affluent smart environments. Through multi-device cooperation and negotiation, the continuous monitoring systems like CoMon~\cite{lee2016comon+} and Remora~\cite{keally2013remora} largely mitigated the main concern of including smartphone users onto the platform. In even more mobile and opportunistic environments, self-organized context neighborhoods \tocheckCL{PINCH}~\cite{liu18:pinch} and \tocheckCL{Stacon}~\cite{liu2019stacon} can be built with low-end sensors and negligible communication overhead. The adoption of these cost-effective continuous sensing systems is improved by these practical enhancements in WSN. It is because of this, our vision of the IoT service personalization can take more context features into account.


\note{\textbf{IoT middleware} connectivity and interoperability in IoT.}



==> rethink_ConAware.tex <==
\section{Rethinking Context-Awareness in the IoT}\label{sec:rethink}
%In this section, we develop a user scenario to rethink how context is leveraged to help people interact with smart devices. Before we start, we \tocheckCJ{\sout{first}} need to categorize the roles of IoT devices \tocheckCJ{we} consider\tocheckCJ{\sout{ed}} in this work as {\em actuators} and {\em sensors}. Actuators are devices to which the user can make requests to take some action (e.g., turn on the lights, adjust the volume, etc. Sensors are devices embedded in the environment to passively collect contextual information. A physical device may take on either role, and can even potentially take on both roles simultaneously. For instance, a smart thermostat can be viewed as a sensor as it can provide temperature readings. The user can also request to change its set point temperature. In the scope of this paper, we will consider devices with both roles as though it is two devices, one with each role.

%We next develop a user scenario that we rely on throughout the paper to motivate and explain our contributions. Alice is a smart home enthusiast. She owns several IoT actuators, including a smart lock, a smart thermostat, a smart lighting system, a smart security system with cameras, and a stereo system. Because she is an early adopter, she purchased these as they became available on the market, so they are naturally provided by five different manufacturers
%\cj{I've corrected this several times, but we want ``manufacturers'' (which is the noun) rather than  ``manufactures'' (which is spelled correctly, but is the verb)}. 
%She also has a networked sensor system deployed throughout her house but by a completely separate provider because it was installed by the construction team when her house was built. The stereo system is her favorite because it supports sophisticated collaboration among all of her speakers to provide \tocheckCL{\sout{perfect} ideal} sound quality. \tocheckCL{As the number of smart devices grow in her house, Alice is trying to figure out a way \sout{Now Alice needs to decide how}} to control all of the devices. In the remainder of this section, we examine what tools Alice has available to her given the current state of the art. We then demonstrate how our approach enables increased personalized automation by leveraging ambient context information and user feedback.\cj{In case you read these notes first, see my comment in the related work about combining (and restructuring) Sections 2 and 3.}


%\begin{figure}[tb]
%\centering
%\begin{subfigure}[b]{.45\columnwidth}
%\includegraphics[width=.99\linewidth]{images/IoT_manufacture.pdf}
%https://docs.google.com/drawings/d/1sqB_OM83G0WvekipL6rA3Il31sbXTiQkH34_GcMiVXE/edit
%\caption{Manufacturer oriented}
%\label{fig:iotManufacture}
%\end{subfigure}
%\begin{subfigure}[b]{.45\columnwidth}
%\includegraphics[width=.99\linewidth]{images/IoT_ind.pdf}
%https://docs.google.com/drawings/d/14a5XR1fkuedKOJOAqN-FDyLHS_ux-H8oC1lQqu5Zx2Q/edit
%\caption{Middleware oriented}
%\label{fig:iotIndividual}
%\end{subfigure}
%\caption{Existing huaman-device interaction in the IoT}
%\label{fig:iotExisting}
%\end{figure}
%\subsection{Existing framework}\label{sec:rethink_exist}
%Fig.~\ref{fig:iotExisting}
% \cj{FYI: I changed the figure to use the subfigure environment rather than the minipage environment. Among other things, this allowed me to align the two subfigures along the bottom.} 
%shows schematics of two existing control options available to Alice. The first, depicted in Fig.~\ref{fig:iotManufacture}, is a manufacturer-oriented view in which Alice controls the actuators through different manufacturer gateways and their (proprietary) applications. The obvious advantage of this approach is that manufacturers are very familiar with their products and can provide comprehensive services. For Alice, this means that she can enjoy all of the features that get her the perfect sound quality from her stereo system. On the other hand, Alice has to navigate the steep and diverse learning curves associated with the control terms and patterns defined by all of the different manufacturers~\cite{landauer1983natural}. Although some manufacturers allow users to define personalized automation (i.e., Nest and Philips Hue) based on primitive context information like time, they cannot leverage the sensor information provided by other manufacturers~\cite{chew2017smart}, and as a result, their smart systems may fail to understand a user's more subtle intentions due to lack of context~\cite{yang2013learning}. In other words, ``personalization'' does not truly reflect the user's preference.\cj{It would seem that a concrete example would really help here.}

%Fig.~\ref{fig:iotIndividual} shows another choice where she can install one IoT middleware that provides universal gateway for all the devices (i.e. IFTTT~\cite{ovadia2014automate}, Hydra~\cite{eisenhauer2010hydra}). In this case, the advantage is that she only need to learn one control language to use all her devices and the contextual data collected by the sensors can also be leveraged. The disadvantage of this approach is that Alice has to define all the interaction pattern by herself under some script language defined by the middleware provider. Even with current context-aware automation solutions (i.e. ~\cite{chahuara2017context, meng2016rule}) incorporated, she would still have to define the rules or semantics. In addition, since the control interfaces are designed by third-party, some features of the devices may not be supported(shown as gray in the Fig.~\ref{fig:iotIndividual}). For example, it is not feasible for a contextual model to coordinate multiple speakers to provide manufacture designed sound effect. 
\begin{figure}[tb]
\centering
\includegraphics[width=.9\columnwidth]{images/Ctx_IoT.pdf}
%https://docs.google.com/drawings/d/1B4Yfg6N0I7v6NmCjZDl-HUpJLcn7zGcaQrYGeCRsiMI/edit
\caption{The overview of the \systemname framework}
\label{fig:iotParadigm}
\end{figure}
\subsection{\systemname framework}\label{sec:rethink_we}
From the previous two examples, we can identify a trade-off between user oriented personalization and manufacture oriented features. We argue that it is important to keep both the user and the manufacture in the loop in order to retain both personalization and full potential of the devices. In Fig.~\ref{fig:iotParadigm}, we propose a novel framework of context-awareness where \systemname is the key to connect the components. In the previous user scenario, all Alice has to do is to issue requests when she want to interact with the devices and give natural feedback to the decision made by \systemname. Built on top of existing middlware, \systemname is able to collect sensor readings and send control command to actuators. When \systemname receives a request, it will tag the request with contextual information and decide which device and what service the user is trying to use. To leverage the domain knowledge from the manufacture, some devices are not directly controlled by \systemname. For example, when Alice issue a request to use the sound system, \systemname will decide based on the context that the user is trying to interact with a external controller, so \systemname will forward the $\langle request,context\rangle$ to the manufacture controller. The manufacture controller is nothing more than a manufacture application with a simple interface implemented to receive context, request and feedback. The personalization is achieved because \systemname framework is a closed loop system, the knowledge by the models is provided by Alice, and thus it's tailored to Alice.

%  \systemname can also cooperate with infrastructure smart assistant in the environment as long as it support the same interface. In this manner, \systemname can push its request to infrastructure assistants and collect results from them which makes the framework more scalable. For example, in smart city setting, public \device{}s may not be able to make one-on-one connection to each user. An infrastructure controller can better leverage different needs from different users while \systemname acts in between to free the user from interacting with different controller manually and provide more personalized experience. Another advantage is that manufacture can provide specialized smart assistant for its devices so that they can leverage the domain knowledge unknown to \systemname to fully exploit the potential of the devices. For example, a specialized sound assistant can control the speakers to provide stereo sound effect and \systemname can control the speakers through this agent.





